Privacy protocols

Security protocols enable secure communication over insecure channels. Privacy protocols enable private interactions over secure channels. Security protocols set up secure channels using cryptographic primitives. Privacy protocols set up private channels using secure channels. But just like some security protocols can be broken without breaking the underlying cryptography, some privacy protocols can be broken without breaking the underlying security. Such privacy attacks have been used to leverage e-commerce against targeted advertising from the outset; but their depth and scope became apparent only with the overwhelming advent of influence campaigns in politics. The blurred boundaries between privacy protocols and privacy attacks present a new challenge for protocol analysis. Covert channels turn out to be concealed not only below overt channels, but also above: subversions, and the level-below attacks are supplemented by sublimations and the level-above attacks.

==> PICS/google-protocol-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Nov 04 17:15:13 CET 2010
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="90" y-min="9.38" y-max="80" auto-bounding="true">
%<ellipse fill-color= "#ccffff"
%	 stroke-width= "0.6"
%	 p3= "(70,10)"
%	 fill-style= "solid"
%	 stroke-color= "#ff3366"
%	 p2= "(70,70)"
%	 p1= "(10,70)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#ffff99"
%	 p3= "(50,30)"
%	 fill-style= "solid"
%	 p2= "(50,50)"
%	 p1= "(30,50)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-width-minimum= "2"
%	 points= "(15,50);(15,50);(39,50);(39,50)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-width-minimum= "2"
%	 points= "(39.37,50);(39.37,50);(39.38,30);(39.38,30)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-width-minimum= "2"
%	 points= "(39,30);(39,30);(14.38,30);(14.38,30)"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45.62,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\indx
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(24.38,50.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\query
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(23.75,30.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\retrieve
%</text>
%<multicurve stroke-width= "0.55"
%	 fill-style= "none"
%	 stroke-color= "#ff3366"
%	 arrow-head-width-minimum= "2"
%	 points= "(90,70);(90,70);(40,70);(40,70)"
%	 right-arrow= "head"
%	 />
%<multicurve stroke-width= "0.55"
%	 fill-style= "none"
%	 stroke-color= "#ff3366"
%	 arrow-head-width-minimum= "2"
%	 points= "(40.12,10);(40.12,10);(90,10);(90,10)"
%	 right-arrow= "head"
%	 />
%<multicurve stroke-width= "0.55"
%	 fill-style= "none"
%	 stroke-color= "#ff3366"
%	 arrow-head-width-minimum= "2"
%	 points= "(40,70);(40,70);(40,10);(40,10)"
%	 right-arrow= "head"
%	 />
%<multicurve stroke-width= "0.55"
%	 fill-style= "none"
%	 stroke-color= "#ff3366"
%	 arrow-head-width-minimum= "2"
%	 points= "(40,29.38);(40,29.38);(12,29.38);(12,29.38)"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(53,52)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\indxx
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(26.25,28.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\supply
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(71.88,69.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\advert
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(71.88,9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\monetize
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\user
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\SE
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(83,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\advertiser
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(90,80)
\newrgbcolor{userLineColour}{1 0.2 0.4}
\newrgbcolor{userFillColour}{0.8 1 1}
\rput{0}(40,40){\psellipse[linewidth=0.6,linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(30,-30)}
\newrgbcolor{userFillColour}{1 1 0.6}
\rput{0}(40,40){\psellipse[fillcolor=userFillColour,fillstyle=solid](0,0)(10,-10)}
\psline[arrowsize=2 2]{->}(15,50)(39,50)
\psline[arrowsize=2 2]{->}(39.37,50)(39.38,30)
\psline[arrowsize=2 2]{->}(39,30)(14.38,30)
\rput(45.62,40){\indx}
\rput[b](24.38,50.62){\query}
\rput[b](23.75,30.62){\retrieve}
\newrgbcolor{userLineColour}{1 0.2 0.4}
\psline[linewidth=0.55,linecolor=userLineColour,arrowsize=2 2]{->}(90,70)(40,70)
\newrgbcolor{userLineColour}{1 0.2 0.4}
\psline[linewidth=0.55,linecolor=userLineColour,arrowsize=2 2]{->}(40.12,10)(90,10)
\newrgbcolor{userLineColour}{1 0.2 0.4}
\psline[linewidth=0.55,linecolor=userLineColour,arrowsize=2 2]{->}(40,70)(40,10)
\newrgbcolor{userLineColour}{1 0.2 0.4}
\psline[linewidth=0.55,linecolor=userLineColour,arrowsize=2 2]{->}(40,29.38)(12,29.38)
\rput(53,52){\indxx}
\rput[t](26.25,28.75){\supply}
\rput[t](71.88,69.38){\advert}
\rput[t](71.88,9.38){\monetize}
\rput(13,80){\user}
\rput(40,80){\SE}
\rput(83,80){\advertiser}
\end{pspicture}


==> PICS/particle.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 10 13:47:07 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="6.25" x-max="75" y-min="5" y-max="30" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(42.5,11.88);(42.5,11.88);(68.12,23.12);(68.12,23.12)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.85"
%	 fill-style= "none"
%	 points= "(36.25,26.25);(36.25,26.25);(67.5,26.25);(67.5,26.25)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 fill-style= "none"
%	 points= "(10.5,25);(10.5,25);(36.88,11.88);(36.88,11.88)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.85"
%	 fill-style= "none"
%	 points= "(11.88,26.25);(11.88,26.25);(30.62,26.25);(30.62,26.25)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<ellipse p3= "(11.5,27)"
%	 p2= "(11.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(8.5,23)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(41.5,12)"
%	 p2= "(41.5,8)"
%	 fill-color= "#ff6666"
%	 p1= "(38.5,8)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(71.5,27)"
%	 p2= "(71.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(68.5,23)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(34.62,28.25)"
%	 p2= "(34.62,24.25)"
%	 fill-color= "#ff6666"
%	 p1= "(31.62,24.25)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Carol
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Alice
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(33.12,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Bob
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(40,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dave
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(75,30)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(42.5,11.88)(68.12,23.12)
\psline[linewidth=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(36.25,26.25)(67.5,26.25)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(10.5,25)(36.88,11.88)
\psline[linewidth=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(11.88,26.25)(30.62,26.25)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(10,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(40,10){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(70,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(33.12,26.25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\rput[l](75,25){\Carol}
\rput[r](6.25,25){\Alice}
\rput[b](33.12,30){\Bob}
\rput[t](40,5){\Dave}
\end{pspicture}


==> PICS/privproc-old.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jan 21 23:56:23 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="198.75" y-min="2.5" y-max="60" auto-bounding="true">
%<multicurve points= "(10,45);(10,45);(60,45);(60,45)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(10,5);(10,5);(60,5);(60,5)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(66.25,40);(66.25,40);(66.25,10);(66.25,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<parallelogram p3= "(67.5,42.5)"
%	 p2= "(67.5,47.5)"
%	 p1= "(62.5,47.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(67.5,2.5)"
%	 p2= "(67.5,7.5)"
%	 p1= "(62.5,7.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(7.5,42.5)"
%	 p2= "(7.5,47.5)"
%	 p1= "(2.5,47.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(7.5,2.5)"
%	 p2= "(7.5,7.5)"
%	 p1= "(2.5,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(35,46.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(35,6.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%$\Response$
%</text>
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "2;2"
%	 points= "(53.75,31.25);(53.75,31.25);(53.75,18.75);(53.75,18.75)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "right"
%	 >
%$\Alceresource$
%</text>
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(63.75,40);(63.75,40);(53.75,31.25);(53.75,31.25)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 stroke-style= "dashed"
%	 arrow-head-width-minimum= "1.5"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(53.75,18.75);(53.75,18.75);(63.75,10);(63.75,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<multicurve points= "(70,45);(70,45);(120,45);(120,45)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(70,5);(70,5);(120,5);(120,5)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<parallelogram p3= "(127.5,42.5)"
%	 p2= "(127.5,47.5)"
%	 p1= "(122.5,47.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(127.5,2.5)"
%	 p2= "(127.5,7.5)"
%	 p1= "(122.5,7.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(130,45);(130,45);(180,45);(180,45)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(130,5);(130,5);(180,5);(180,5)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<parallelogram p3= "(187.5,42.5)"
%	 p2= "(187.5,47.5)"
%	 p1= "(182.5,47.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(187.5,2.5)"
%	 p2= "(187.5,7.5)"
%	 p1= "(182.5,7.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(95,46.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RequestBC$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(95,6.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ResponseBC$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.75,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BobresourceR$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(112.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Carolresource$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(125,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Carol
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(185,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dave
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(127.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\CarolresourceR$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(172.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Daveresource$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(155,46.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RequestCD$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(155,6.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ResponseCD$
%</text>
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(3.75,40);(3.75,40);(3.75,10);(3.75,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\AlceresourceR$
%</text>
%<multicurve stroke-dotsep= "2"
%	 stroke-style= "dotted"
%	 points= "(191.25,45);(191.25,45);(198.75,45);(198.75,45)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-dotsep= "2"
%	 stroke-style= "dotted"
%	 points= "(191.25,5);(191.25,5);(198.75,5);(198.75,5)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(60,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\union$
%</text>
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(126.25,40);(126.25,40);(126.25,10);(126.25,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "2;2"
%	 points= "(113.75,31.25);(113.75,31.25);(113.75,18.75);(113.75,18.75)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(123.75,40);(123.75,40);(113.75,31.25);(113.75,31.25)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 stroke-style= "dashed"
%	 arrow-head-width-minimum= "1.5"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(113.75,18.75);(113.75,18.75);(123.75,10);(123.75,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(120,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\union$
%</text>
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(186.25,40);(186.25,40);(186.25,10);(186.25,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "2;2"
%	 points= "(173.75,31.25);(173.75,31.25);(173.75,18.75);(173.75,18.75)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(183.75,40);(183.75,40);(173.75,31.25);(173.75,31.25)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 stroke-style= "dashed"
%	 arrow-head-width-minimum= "1.5"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(173.75,18.75);(173.75,18.75);(183.75,10);(183.75,10)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(180,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\union$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(187.5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DaveresourceR$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(198.75,60)
\psline[linewidth=0.65,arrowinset=0]{<-}(10,45)(60,45)
\psline[linewidth=0.65,arrowinset=0]{->}(10,5)(60,5)
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(66.25,40)(66.25,10)
\pspolygon[](62.5,47.5)(67.5,47.5)(67.5,42.5)(62.5,42.5)
\pspolygon[](62.5,7.5)(67.5,7.5)(67.5,2.5)(62.5,2.5)
\pspolygon[](2.5,47.5)(7.5,47.5)(7.5,42.5)(2.5,42.5)
\pspolygon[](2.5,7.5)(7.5,7.5)(7.5,2.5)(2.5,2.5)
\rput(5,60){\Alce}
\rput(65,60){\Bobo}
\rput[b](35,46.25){$\Request$}
\rput[b](35,6.25){$\Response$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](53.75,31.25)(53.75,18.75)
\rput[r](2.5,25){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8](63.75,40)(53.75,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(53.75,18.75)(63.75,10)
\psline[linewidth=0.65,arrowinset=0]{<-}(70,45)(120,45)
\psline[linewidth=0.65,arrowinset=0]{->}(70,5)(120,5)
\pspolygon[](122.5,47.5)(127.5,47.5)(127.5,42.5)(122.5,42.5)
\pspolygon[](122.5,7.5)(127.5,7.5)(127.5,2.5)(122.5,2.5)
\psline[linewidth=0.65,arrowinset=0]{<-}(130,45)(180,45)
\psline[linewidth=0.65,arrowinset=0]{->}(130,5)(180,5)
\pspolygon[](182.5,47.5)(187.5,47.5)(187.5,42.5)(182.5,42.5)
\pspolygon[](182.5,7.5)(187.5,7.5)(187.5,2.5)(182.5,2.5)
\rput[b](95,46.25){$\RequestBC$}
\rput[b](95,6.25){$\ResponseBC$}
\rput[l](68.75,25){$\BobresourceR$}
\rput[r](112.5,25){$\Carolresource$}
\rput(125,60){\Carol}
\rput(185,60){\Dave}
\rput[l](127.5,25){$\CarolresourceR$}
\rput[r](172.5,25){$\Daveresource$}
\rput[b](155,46.25){$\RequestCD$}
\rput[b](155,6.25){$\ResponseCD$}
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(3.75,40)(3.75,10)
\rput[r](51.25,25){$\AlceresourceR$}
\psline[linewidth=0.65,linestyle=dotted,dotsep=2](191.25,45)(198.75,45)
\psline[linewidth=0.65,linestyle=dotted,dotsep=2](191.25,5)(198.75,5)
\rput(60,25){$\union$}
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(126.25,40)(126.25,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](113.75,31.25)(113.75,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8](123.75,40)(113.75,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(113.75,18.75)(123.75,10)
\rput(120,25){$\union$}
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(186.25,40)(186.25,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](173.75,31.25)(173.75,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8](183.75,40)(173.75,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(173.75,18.75)(183.75,10)
\rput(180,25){$\union$}
\rput[l](187.5,25){$\DaveresourceR$}
\end{pspicture}


==> PICS/privproc.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Feb 08 04:06:14 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="12.5" x-max="121.25" y-min="3.75" y-max="80" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(50,45);(50,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(50,5);(50,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(55,40);(55,40);(55,10);(55,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(56.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(25,31.25);(25,31.25);(25,18.75);(25,18.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(16.25,40);(16.25,40);(25,31.25);(25,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(25,18.75);(25,18.75);(16.25,10);(16.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(13.75,40);(13.75,40);(13.75,10);(13.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,46.25);(47.5,46.25);(50,45);(50,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(22.5,3.75);(22.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(85,65);(85,65);(115,65);(115,65)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,25);(85,25);(115,25);(115,25)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(120,60);(120,60);(120,30);(120,30)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.45"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(100,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(100,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(121.25,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(90,51.25);(90,51.25);(90,38.75);(90,38.75)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(77.5,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(81.25,60);(81.25,60);(90,51.25);(90,51.25)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(90,38.75);(90,38.75);(81.25,30);(81.25,30)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.45"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(78.75,60);(78.75,60);(78.75,30);(78.75,30)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.45"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(112.5,66.25);(112.5,66.25);(115,65);(115,65)"
%	 stroke-width= "0.45"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,25);(85,25);(87.5,23.75);(87.5,23.75)"
%	 stroke-width= "0.45"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(91.25,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(120,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(80,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(85,45.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.45"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(121.25,80)
\psline[linewidth=0.65](20,45)(50,45)
\psline[linewidth=0.65](20,5)(50,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(55,40)(55,10)
\rput(15,60){\Alce}
\rput(55,60){\Bobo}
\rput[b](35,46.25){$\Request$}
\rput[b](35,6.25){$\Response$}
\rput[l](56.25,25){$\Bobsresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](25,31.25)(25,18.75)
\rput[r](12.5,25){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](16.25,40)(25,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(25,18.75)(16.25,10)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(13.75,40)(13.75,10)
\psline[linewidth=0.65](47.5,46.25)(50,45)
\psline[linewidth=0.65](20,5)(22.5,3.75)
\rput[l](26.25,25){$\Alcebobsresource$}
\rput(55,45){\Vars}
\rput(15,5){\Vals}
\rput(55,5){\Vals}
\rput(15,45){\Vars}
\rput(20,25.62){$\addjoin$}
\psline[linewidth=0.45](85,65)(115,65)
\psline[linewidth=0.45](85,25)(115,25)
\psline[linewidth=0.45,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(120,60)(120,30)
\rput(80,80){\Alce}
\rput(120,80){\Bobo}
\rput[b](100,66.25){$\Request$}
\rput[b](100,26.25){$\Response$}
\rput[l](121.25,45){$\Bobsresource$}
\psline[linewidth=0.45,linestyle=dashed,dash=2 2](90,51.25)(90,38.75)
\rput[r](77.5,45){$\Alceresource$}
\psline[linewidth=0.45,linestyle=dashed,dash=2 2](81.25,60)(90,51.25)
\psline[linewidth=0.45,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(90,38.75)(81.25,30)
\psline[linewidth=0.45,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(78.75,60)(78.75,30)
\psline[linewidth=0.45](112.5,66.25)(115,65)
\psline[linewidth=0.45](85,25)(87.5,23.75)
\rput[l](91.25,45){$\Alcebobsresource$}
\rput(120,65){\Vars}
\rput(80,25){\Vals}
\rput(120,25){\Vals}
\rput(80,65){\Vars}
\rput(85,45.62){$\addjoin$}
\end{pspicture}


==> PICS/privwave-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jan 23 13:57:33 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="108.75" y-min="12.5" y-max="170" auto-bounding="true">
%<multicurve points= "(10,100);(10,100);(60,150);(60,150)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(10,60);(10,60);(60,110);(60,110)"
%	 fill-style= "none"
%	 stroke-width= "0.5"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(66.25,150);(66.25,150);(66.25,120);(66.25,120)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<parallelogram p3= "(67.5,152.5)"
%	 p2= "(67.5,157.5)"
%	 p1= "(62.5,157.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(67.5,112.5)"
%	 p2= "(67.5,117.5)"
%	 p1= "(62.5,117.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(7.5,92.5)"
%	 p2= "(7.5,97.5)"
%	 p1= "(2.5,97.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(7.5,52.5)"
%	 p2= "(7.5,57.5)"
%	 p1= "(2.5,57.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,110)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,170)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(22.5,116.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(47.5,102.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "center-h"
%	 >
%$\Response$
%</text>
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "2;2"
%	 points= "(60,145);(60,145);(60,125);(60,125)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(2.5,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 right-arrow= "head"
%	 text-hor-align= "right"
%	 >
%$\Alceresource$
%</text>
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(63.75,150);(63.75,150);(60,145);(60,145)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 stroke-style= "dashed"
%	 arrow-head-width-minimum= "1.5"
%	 stroke-dasharray= "1.2;2.8"
%	 points= "(60,125);(60,125);(63.75,120);(63.75,120)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<multicurve points= "(70,150);(70,150);(100,120);(100,120)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(70,110);(70,110);(100,80);(100,80)"
%	 fill-style= "none"
%	 stroke-width= "0.5"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<parallelogram p3= "(107.5,112.5)"
%	 p2= "(107.5,117.5)"
%	 p1= "(102.5,117.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(107.5,72.5)"
%	 p2= "(107.5,77.5)"
%	 p1= "(102.5,77.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-overstrike-width= "1.5"
%	 stroke-overstrike= "true"
%	 points= "(10,90);(10,90);(40,60);(40,60)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve points= "(10,50);(10,50);(40,20);(40,20)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<parallelogram p3= "(47.5,52.5)"
%	 p2= "(47.5,57.5)"
%	 p1= "(42.5,57.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(47.5,12.5)"
%	 p2= "(47.5,17.5)"
%	 p1= "(42.5,17.5)"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(80,143.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RequestBC$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.75,135)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\BobresourceR$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(38.75,36.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Carolresource$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Carol
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(105,130)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dave
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(48.75,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\CarolresourceR$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(90,103.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\RequestCD$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(87.5,61.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ResponseCD$
%</text>
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(3.75,90);(3.75,90);(3.75,60);(3.75,60)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(63.12,135)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\union$
%</text>
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(106.25,110);(106.25,110);(106.25,80);(106.25,80)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<multicurve arrow-head-length-scale= "1.5"
%	 arrow-head-width-minimum= "1.5"
%	 points= "(46.25,50);(46.25,50);(46.25,20);(46.25,20)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0.05"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(108.75,95)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DaveresourceR$
%</text>
%<multicurve points= "(50,20);(50,20);(100,70);(100,70)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%<multicurve stroke-overstrike-width= "1.5"
%	 stroke-overstrike= "true"
%	 points= "(50,60);(50,60);(100,110);(100,110)"
%	 fill-style= "none"
%	 stroke-width= "0.65"
%	 left-arrow= "head"
%	 arrow-head-inset-scale= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(108.75,170)
\psline[linewidth=0.65,arrowinset=0]{<-}(10,100)(60,150)
\psline[linewidth=0.5,arrowinset=0]{->}(10,60)(60,110)
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(66.25,150)(66.25,120)
\pspolygon[](62.5,157.5)(67.5,157.5)(67.5,152.5)(62.5,152.5)
\pspolygon[](62.5,117.5)(67.5,117.5)(67.5,112.5)(62.5,112.5)
\pspolygon[](2.5,97.5)(7.5,97.5)(7.5,92.5)(2.5,92.5)
\pspolygon[](2.5,57.5)(7.5,57.5)(7.5,52.5)(2.5,52.5)
\rput(5,110){\Alce}
\rput(65,170){\Bobo}
\rput[b](22.5,116.25){$\Request$}
\rput[b](47.5,102.5){$\Response$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](60,145)(60,125)
\rput[r](2.5,75){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8](63.75,150)(60,145)
\psline[linewidth=0.65,linestyle=dashed,dash=1.2 2.8,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(60,125)(63.75,120)
\psline[linewidth=0.65,arrowinset=0]{<-}(70,150)(100,120)
\psline[linewidth=0.5,arrowinset=0]{->}(70,110)(100,80)
\pspolygon[](102.5,117.5)(107.5,117.5)(107.5,112.5)(102.5,112.5)
\pspolygon[](102.5,77.5)(107.5,77.5)(107.5,72.5)(102.5,72.5)
\psline[linewidth=0.65,border=1.5,arrowinset=0]{<-}(10,90)(40,60)
\psline[linewidth=0.65,arrowinset=0]{->}(10,50)(40,20)
\pspolygon[](42.5,57.5)(47.5,57.5)(47.5,52.5)(42.5,52.5)
\pspolygon[](42.5,17.5)(47.5,17.5)(47.5,12.5)(42.5,12.5)
\rput[b](80,143.75){$\RequestBC$}
\rput[l](68.75,135){$\BobresourceR$}
\rput[r](38.75,36.25){$\Carolresource$}
\rput(45,70){\Carol}
\rput(105,130){\Dave}
\rput[l](48.75,35){$\CarolresourceR$}
\rput[b](90,103.75){$\RequestCD$}
\rput[b](87.5,61.25){$\ResponseCD$}
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(3.75,90)(3.75,60)
\rput(63.12,135){$\union$}
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(106.25,110)(106.25,80)
\psline[linewidth=0.65,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(46.25,50)(46.25,20)
\rput[l](108.75,95){$\DaveresourceR$}
\psline[linewidth=0.65,arrowinset=0]{->}(50,20)(100,70)
\psline[linewidth=0.65,border=1.5,arrowinset=0]{<-}(50,60)(100,110)
\end{pspicture}


==> PICS/privwave-old.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Feb 08 20:22:20 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="12.5" x-max="136.25" y-min="3.75" y-max="80" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,45);(20,45);(50,45);(50,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(50,5);(50,5)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(35,42.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(35,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(25,31.25);(25,31.25);(25,18.75);(25,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(16.25,40);(16.25,40);(25,31.25);(25,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(25,18.75);(25,18.75);(16.25,10);(16.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(13.75,40);(13.75,40);(13.75,10);(13.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(47.5,46.25);(47.5,46.25);(50,45);(50,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(22.5,3.75);(22.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(100,65);(100,65);(130,65);(130,65)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,25);(100,25);(130,25);(130,25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(135,60);(135,60);(135,30);(135,30)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.6"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,80)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(115,66.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(115,26.25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(92.5,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(105,51.25);(105,51.25);(105,38.75);(105,38.75)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(136.25,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(96.25,60);(96.25,60);(105,51.25);(105,51.25)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(105,38.75);(105,38.75);(96.25,30);(96.25,30)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.35"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(93.75,60);(93.75,60);(93.75,30);(93.75,30)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.35"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(127.5,66.25);(127.5,66.25);(130,65);(130,65)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(100,25);(100,25);(102.5,23.75);(102.5,23.75)"
%	 stroke-width= "0.35"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(106.25,45)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(135,25)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(95,65)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,45.62)"
%	 text-frame= "noframe"
%	 stroke-width= "0.35"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20,46.25);(20,46.25);(90,63.12);(90,63.12)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(86.88,63.75);(86.88,63.75);(90,63.12);(90,63.12)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 stroke-overstrike-width= "1.5"
%	 points= "(61.25,45);(61.25,45);(130,61.88);(130,61.88)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(126.88,62.5);(126.88,62.5);(130,61.88);(130,61.88)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(60,5.62);(60,5.62);(128.75,22.5);(128.75,22.5)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(126.88,23.12);(126.88,23.12);(130,22.5);(130,22.5)"
%	 stroke-width= "0.6"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20,7.5);(20,7.5);(88.75,24.38);(88.75,24.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(86.25,25);(86.25,25);(89.38,24.38);(89.38,24.38)"
%	 stroke-width= "0.35"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(56.88,53.12);(56.88,53.12);(80.62,58.12);(80.62,58.12)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(44.38,48.12);(44.38,48.12);(75.62,51.88);(75.62,51.88)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,46.88);(27.5,46.88);(57.5,53.12);(57.5,53.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(29.38,46.25);(29.38,46.25);(59.38,50);(59.38,50)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(105,61.88);(105,61.88);(121.88,63.12);(121.88,63.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(106.88,58.75);(106.88,58.75);(121.88,61.88);(121.88,61.88)"
%	 stroke-width= "0.35"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(96.88,61.25);(96.88,61.25);(106.88,61.88);(106.88,61.88)"
%	 stroke-width= "0.4"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(82.5,53.75);(82.5,53.75);(112.5,60);(112.5,60)"
%	 stroke-width= "0.4"
%	 />
%<multicurve fill-style= "none"
%	 points= "(119.38,63.75);(119.38,63.75);(121.88,63.12);(121.88,63.12)"
%	 stroke-width= "0.35"
%	 />
%<multicurve fill-style= "none"
%	 points= "(119.38,61.88);(119.38,61.88);(121.88,61.88);(121.88,61.88)"
%	 stroke-width= "0.35"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(56.25,13.12);(56.25,13.12);(80,18.12);(80,18.12)"
%	 stroke-width= "0.25"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(43.75,8.12);(43.75,8.12);(75,11.88);(75,11.88)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.88,6.88);(26.88,6.88);(56.88,13.12);(56.88,13.12)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.75,6.25);(28.75,6.25);(58.75,10);(58.75,10)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(104.38,21.88);(104.38,21.88);(121.25,23.12);(121.25,23.12)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(106.25,18.75);(106.25,18.75);(121.25,21.88);(121.25,21.88)"
%	 stroke-width= "0.25"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(96.25,21.25);(96.25,21.25);(106.25,21.88);(106.25,21.88)"
%	 stroke-width= "0.25"
%	 />
%<multicurve stroke-dotsep= "2"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(81.88,13.75);(81.88,13.75);(111.88,20);(111.88,20)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(118.75,23.75);(118.75,23.75);(121.25,23.12);(121.25,23.12)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 points= "(118.75,21.88);(118.75,21.88);(121.25,21.88);(121.25,21.88)"
%	 stroke-width= "0.25"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 stroke-overstrike-width= "1.5"
%	 points= "(53.75,40);(53.75,40);(53.75,9.38);(53.75,9.38)"
%	 arrow-head-width-minimum= "1.55"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Carol
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dave
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-overstrike-width= "1"
%	 stroke-style= "dashed"
%	 points= "(65,31.25);(65,31.25);(65,18.75);(65,18.75)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-overstrike-width= "1"
%	 stroke-style= "dashed"
%	 points= "(56.25,40);(56.25,40);(65,31.25);(65,31.25)"
%	 stroke-overstrike= "true"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-overstrike-width= "1"
%	 stroke-style= "dashed"
%	 points= "(65,18.75);(65,18.75);(56.25,10);(56.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(60,25.62)"
%	 stroke-overstrike-width= "1"
%	 text-frame= "noframe"
%	 stroke-overstrike= "true"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(12.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Davesresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(26.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DaveBobCarolResource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\CarolAliceResource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(52.5,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\CarolsResource$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(136.25,80)
\psline[linewidth=0.65](20,45)(50,45)
\psline[linewidth=0.65](20,5)(50,5)
\rput[t](35,42.5){$\Request$}
\rput[t](35,3.75){$\Response$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](25,31.25)(25,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](16.25,40)(25,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(25,18.75)(16.25,10)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(13.75,40)(13.75,10)
\psline[linewidth=0.65](47.5,46.25)(50,45)
\psline[linewidth=0.65](20,5)(22.5,3.75)
\rput(55,45){\Vars}
\rput(15,5){\Vals}
\rput(55,5){\Vals}
\rput(15,45){\Vars}
\rput(20,25.62){$\addjoin$}
\psline[linewidth=0.6](100,65)(130,65)
\psline[linewidth=0.35](100,25)(130,25)
\psline[linewidth=0.6,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(135,60)(135,30)
\rput(135,80){\Alce}
\rput(95,80){\Bobo}
\rput[b](115,66.25){$\Request$}
\rput[b](115,26.25){$\Response$}
\rput[r](92.5,45){$\Bobsresource$}
\psline[linewidth=0.35,linestyle=dashed,dash=2 2](105,51.25)(105,38.75)
\rput[l](136.25,45){$\Alceresource$}
\psline[linewidth=0.35,linestyle=dashed,dash=2 2](96.25,60)(105,51.25)
\psline[linewidth=0.35,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(105,38.75)(96.25,30)
\psline[linewidth=0.35,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(93.75,60)(93.75,30)
\psline[linewidth=0.6](127.5,66.25)(130,65)
\psline[linewidth=0.35](100,25)(102.5,23.75)
\rput[l](106.25,45){$\Alcebobsresource$}
\rput(135,65){\Vars}
\rput(95,25){\Vals}
\rput(135,25){\Vals}
\rput(95,65){\Vars}
\rput(100,45.62){$\addjoin$}
\psline[linewidth=0.6](20,46.25)(90,63.12)
\psline[linewidth=0.6](86.88,63.75)(90,63.12)
\psline[linewidth=0.6,border=1.5](61.25,45)(130,61.88)
\psline[linewidth=0.6](126.88,62.5)(130,61.88)
\psline[linewidth=0.6](60,5.62)(128.75,22.5)
\psline[linewidth=0.6](126.88,23.12)(130,22.5)
\psline[linewidth=0.35](20,7.5)(88.75,24.38)
\psline[linewidth=0.35](86.25,25)(89.38,24.38)
\psline[linewidth=0.4,linestyle=dotted,dotsep=2](56.88,53.12)(80.62,58.12)
\psline[linewidth=0.4,linestyle=dotted,dotsep=2](44.38,48.12)(75.62,51.88)
\psline[linewidth=0.35](27.5,46.88)(57.5,53.12)
\psline[linewidth=0.35](29.38,46.25)(59.38,50)
\psline[linewidth=0.35](105,61.88)(121.88,63.12)
\psline[linewidth=0.35](106.88,58.75)(121.88,61.88)
\psline[linewidth=0.4,linestyle=dotted,dotsep=2](96.88,61.25)(106.88,61.88)
\psline[linewidth=0.4,linestyle=dotted,dotsep=2](82.5,53.75)(112.5,60)
\psline[linewidth=0.35](119.38,63.75)(121.88,63.12)
\psline[linewidth=0.35](119.38,61.88)(121.88,61.88)
\psline[linewidth=0.25,linestyle=dotted,dotsep=2](56.25,13.12)(80,18.12)
\psline[linewidth=0.25,linestyle=dotted,dotsep=2](43.75,8.12)(75,11.88)
\psline[linewidth=0.25](26.88,6.88)(56.88,13.12)
\psline[linewidth=0.25](28.75,6.25)(58.75,10)
\psline[linewidth=0.25](104.38,21.88)(121.25,23.12)
\psline[linewidth=0.25](106.25,18.75)(121.25,21.88)
\psline[linewidth=0.25,linestyle=dotted,dotsep=2](96.25,21.25)(106.25,21.88)
\psline[linewidth=0.25,linestyle=dotted,dotsep=2](81.88,13.75)(111.88,20)
\psline[linewidth=0.25](118.75,23.75)(121.25,23.12)
\psline[linewidth=0.25](118.75,21.88)(121.25,21.88)
\psline[linewidth=0.65,border=1.5,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(53.75,40)(53.75,9.38)
\rput(55,80){\Carol}
\rput(15,80){\Dave}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,border=1](65,31.25)(65,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,border=1](56.25,40)(65,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,border=1,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(65,18.75)(56.25,10)
\rput(60,25.62){$\addjoin$}
\rput[r](12.5,25){$\Davesresource$}
\rput[l](26.25,25){$\DaveBobCarolResource$}
\rput[l](66.25,25){$\CarolAliceResource$}
\rput[r](52.5,23.75){$\CarolsResource$}
\end{pspicture}


==> PICS/tracking-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Feb 07 06:22:44 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="210" y-min="3.75" y-max="135" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(60,45);(60,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(60,5);(60,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(63.75,40);(63.75,40);(63.75,10);(63.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,31.25);(15,31.25);(15,18.75);(15,18.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(6.25,40);(6.25,40);(15,31.25);(15,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,18.75);(15,18.75);(6.25,10);(6.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(3.75,40);(3.75,40);(3.75,10);(3.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,46.25);(57.5,46.25);(60,45);(60,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(12.5,3.75);(12.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(120,45);(120,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,5);(70,5);(120,5);(120,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(123.75,40);(123.75,40);(123.75,10);(123.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,31.25);(75,31.25);(75,18.75);(75,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(66.25,40);(66.25,40);(75,31.25);(75,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,18.75);(75,18.75);(66.25,10);(66.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,46.25);(117.5,46.25);(120,45);(120,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,5);(70,5);(72.5,3.75);(72.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,45);(130,45);(180,45);(180,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,5);(130,5);(180,5);(180,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(183.75,40);(183.75,40);(183.75,10);(183.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,31.25);(135,31.25);(135,18.75);(135,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(126.25,40);(126.25,40);(135,31.25);(135,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,18.75);(135,18.75);(126.25,10);(126.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,46.25);(177.5,46.25);(180,45);(180,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,5);(130,5);(132.5,3.75);(132.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,45);(190,45);(210,45);(210,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,5);(190,5);(210,5);(210,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,31.25);(195,31.25);(195,18.75);(195,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(186.25,40);(186.25,40);(195,31.25);(195,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,18.75);(195,18.75);(186.25,10);(186.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,120);(10,120);(60,120);(60,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(60,80);(60,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(63.75,115);(63.75,115);(63.75,85);(63.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,106.25);(15,106.25);(15,93.75);(15,93.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(6.25,115);(6.25,115);(15,106.25);(15,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,93.75);(15,93.75);(6.25,85);(6.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(3.75,115);(3.75,115);(3.75,85);(3.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,121.25);(57.5,121.25);(60,120);(60,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(12.5,78.75);(12.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,120);(70,120);(120,120);(120,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(120,80);(120,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(123.75,115);(123.75,115);(123.75,85);(123.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,106.25);(75,106.25);(75,93.75);(75,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(66.25,115);(66.25,115);(75,106.25);(75,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,93.75);(75,93.75);(66.25,85);(66.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,121.25);(117.5,121.25);(120,120);(120,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(72.5,78.75);(72.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,120);(130,120);(180,120);(180,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,80);(130,80);(180,80);(180,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(183.75,115);(183.75,115);(183.75,85);(183.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,106.25);(135,106.25);(135,93.75);(135,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(126.25,115);(126.25,115);(135,106.25);(135,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,93.75);(135,93.75);(126.25,85);(126.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,121.25);(177.5,121.25);(180,120);(180,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,80);(130,80);(132.5,78.75);(132.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,120);(190,120);(210,120);(210,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,80);(190,80);(210,80);(210,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,106.25);(195,106.25);(195,93.75);(195,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(186.25,115);(186.25,115);(195,106.25);(195,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,93.75);(195,93.75);(186.25,85);(186.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(210,135)
\psline[linewidth=0.65](10,45)(60,45)
\psline[linewidth=0.65](10,5)(60,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(63.75,40)(63.75,10)
\rput(5,60){\Alce}
\rput(65,60){\Bobo}
\rput[b](35,46.25){$\Request$}
\rput[b](35,6.25){$\Response$}
\rput[r](62.5,25){$\Bobsresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](15,31.25)(15,18.75)
\rput[r](2.5,25){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](6.25,40)(15,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(15,18.75)(6.25,10)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(3.75,40)(3.75,10)
\psline[linewidth=0.65](57.5,46.25)(60,45)
\psline[linewidth=0.65](10,5)(12.5,3.75)
\rput[l](16.25,25){$\Alcebobsresource$}
\rput(65,45){\Vars}
\rput(5,5){\Vals}
\rput(65,5){\Vals}
\rput(5,45){\Vars}
\rput(10,25.62){$\addjoin$}
\psline[linewidth=0.65](70,45)(120,45)
\psline[linewidth=0.65](70,5)(120,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(123.75,40)(123.75,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](75,31.25)(75,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](66.25,40)(75,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(75,18.75)(66.25,10)
\psline[linewidth=0.65](117.5,46.25)(120,45)
\psline[linewidth=0.65](70,5)(72.5,3.75)
\rput(125,45){\Vars}
\rput(125,5){\Vals}
\rput(70,25.62){$\addjoin$}
\psline[linewidth=0.65](130,45)(180,45)
\psline[linewidth=0.65](130,5)(180,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(183.75,40)(183.75,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](135,31.25)(135,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](126.25,40)(135,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(135,18.75)(126.25,10)
\psline[linewidth=0.65](177.5,46.25)(180,45)
\psline[linewidth=0.65](130,5)(132.5,3.75)
\rput(185,45){\Vars}
\rput(185,5){\Vals}
\rput(130,25.62){$\addjoin$}
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,45)(210,45)
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,5)(210,5)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](195,31.25)(195,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](186.25,40)(195,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(195,18.75)(186.25,10)
\rput(190,25.62){$\addjoin$}
\psline[linewidth=0.65](10,120)(60,120)
\psline[linewidth=0.65](10,80)(60,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(63.75,115)(63.75,85)
\rput(5,135){\Alce}
\rput(65,135){\Bobo}
\rput[b](35,121.25){$\Request$}
\rput[b](35,81.25){$\Response$}
\rput[r](62.5,100){$\Bobsresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](15,106.25)(15,93.75)
\rput[r](2.5,100){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](6.25,115)(15,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(15,93.75)(6.25,85)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(3.75,115)(3.75,85)
\psline[linewidth=0.65](57.5,121.25)(60,120)
\psline[linewidth=0.65](10,80)(12.5,78.75)
\rput[l](16.25,100){$\Alcebobsresource$}
\rput(65,120){\Vars}
\rput(5,80){\Vals}
\rput(65,80){\Vals}
\rput(5,120){\Vars}
\rput(10,100.62){$\addjoin$}
\psline[linewidth=0.65](70,120)(120,120)
\psline[linewidth=0.65](70,80)(120,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(123.75,115)(123.75,85)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](75,106.25)(75,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](66.25,115)(75,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(75,93.75)(66.25,85)
\psline[linewidth=0.65](117.5,121.25)(120,120)
\psline[linewidth=0.65](70,80)(72.5,78.75)
\rput(125,120){\Vars}
\rput(125,80){\Vals}
\rput(70,100.62){$\addjoin$}
\psline[linewidth=0.65](130,120)(180,120)
\psline[linewidth=0.65](130,80)(180,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(183.75,115)(183.75,85)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](135,106.25)(135,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](126.25,115)(135,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(135,93.75)(126.25,85)
\psline[linewidth=0.65](177.5,121.25)(180,120)
\psline[linewidth=0.65](130,80)(132.5,78.75)
\rput(185,120){\Vars}
\rput(185,80){\Vals}
\rput(130,100.62){$\addjoin$}
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,120)(210,120)
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,80)(210,80)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](195,106.25)(195,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](186.25,115)(195,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(195,93.75)(186.25,85)
\rput(190,100.62){$\addjoin$}
\end{pspicture}


==> PICS/tracking.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Feb 07 01:06:15 GMT-10:00 2019
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="2.5" x-max="210" y-min="3.75" y-max="135" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(10,45);(10,45);(60,45);(60,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(60,5);(60,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(63.75,40);(63.75,40);(63.75,10);(63.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,60)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,46.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,31.25);(15,31.25);(15,18.75);(15,18.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(6.25,40);(6.25,40);(15,31.25);(15,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,18.75);(15,18.75);(6.25,10);(6.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(3.75,40);(3.75,40);(3.75,10);(3.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,46.25);(57.5,46.25);(60,45);(60,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,5);(10,5);(12.5,3.75);(12.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,45);(70,45);(120,45);(120,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,5);(70,5);(120,5);(120,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(123.75,40);(123.75,40);(123.75,10);(123.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,31.25);(75,31.25);(75,18.75);(75,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(66.25,40);(66.25,40);(75,31.25);(75,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,18.75);(75,18.75);(66.25,10);(66.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,46.25);(117.5,46.25);(120,45);(120,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,5);(70,5);(72.5,3.75);(72.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,45);(130,45);(180,45);(180,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,5);(130,5);(180,5);(180,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(183.75,40);(183.75,40);(183.75,10);(183.75,10)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,31.25);(135,31.25);(135,18.75);(135,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(126.25,40);(126.25,40);(135,31.25);(135,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,18.75);(135,18.75);(126.25,10);(126.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,46.25);(177.5,46.25);(180,45);(180,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,5);(130,5);(132.5,3.75);(132.5,3.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,45);(190,45);(210,45);(210,45)"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,5);(190,5);(210,5);(210,5)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,31.25);(195,31.25);(195,18.75);(195,18.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(186.25,40);(186.25,40);(195,31.25);(195,31.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,18.75);(195,18.75);(186.25,10);(186.25,10)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,25.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,120);(10,120);(60,120);(60,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(60,80);(60,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(63.75,115);(63.75,115);(63.75,85);(63.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Alce
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,135)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%\Bobo
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,121.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Request$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(35,81.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 right-arrow= "head"
%	 >
%$\Response$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(62.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Bobsresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,106.25);(15,106.25);(15,93.75);(15,93.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(2.5,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 right-arrow= "head"
%	 >
%$\Alceresource$
%</text>
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(6.25,115);(6.25,115);(15,106.25);(15,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(15,93.75);(15,93.75);(6.25,85);(6.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(3.75,115);(3.75,115);(3.75,85);(3.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(57.5,121.25);(57.5,121.25);(60,120);(60,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,80);(10,80);(12.5,78.75);(12.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,100)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Alcebobsresource$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(70,120);(70,120);(120,120);(120,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(120,80);(120,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(123.75,115);(123.75,115);(123.75,85);(123.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,106.25);(75,106.25);(75,93.75);(75,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(66.25,115);(66.25,115);(75,106.25);(75,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(75,93.75);(75,93.75);(66.25,85);(66.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(117.5,121.25);(117.5,121.25);(120,120);(120,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(70,80);(70,80);(72.5,78.75);(72.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(125,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve fill-style= "none"
%	 points= "(130,120);(130,120);(180,120);(180,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,80);(130,80);(180,80);(180,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0"
%	 points= "(183.75,115);(183.75,115);(183.75,85);(183.75,85)"
%	 arrow-head-width-minimum= "1.55"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,106.25);(135,106.25);(135,93.75);(135,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(126.25,115);(126.25,115);(135,106.25);(135,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(135,93.75);(135,93.75);(126.25,85);(126.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(177.5,121.25);(177.5,121.25);(180,120);(180,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 points= "(130,80);(130,80);(132.5,78.75);(132.5,78.75)"
%	 stroke-width= "0.65"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,120)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vars
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(185,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Vals
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(130,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,120);(190,120);(210,120);(210,120)"
%	 stroke-width= "0.65"
%	 />
%<multicurve stroke-dotsep= "4"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(190,80);(190,80);(210,80);(210,80)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,106.25);(195,106.25);(195,93.75);(195,93.75)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(186.25,115);(186.25,115);(195,106.25);(195,106.25)"
%	 stroke-width= "0.65"
%	 />
%<multicurve fill-style= "none"
%	 arrow-head-inset-scale= "0.05"
%	 stroke-dasharray= "2;2"
%	 stroke-style= "dashed"
%	 points= "(195,93.75);(195,93.75);(186.25,85);(186.25,85)"
%	 arrow-head-width-minimum= "1.5"
%	 arrow-head-length-scale= "1.5"
%	 stroke-width= "0.65"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(190,100.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\addjoin$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(210,135)
\psline[linewidth=0.65](10,45)(60,45)
\psline[linewidth=0.65](10,5)(60,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(63.75,40)(63.75,10)
\rput(5,60){\Alce}
\rput(65,60){\Bobo}
\rput[b](35,46.25){$\Request$}
\rput[b](35,6.25){$\Response$}
\rput[r](62.5,25){$\Bobsresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](15,31.25)(15,18.75)
\rput[r](2.5,25){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](6.25,40)(15,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(15,18.75)(6.25,10)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(3.75,40)(3.75,10)
\psline[linewidth=0.65](57.5,46.25)(60,45)
\psline[linewidth=0.65](10,5)(12.5,3.75)
\rput[l](16.25,25){$\Alcebobsresource$}
\rput(65,45){\Vars}
\rput(5,5){\Vals}
\rput(65,5){\Vals}
\rput(5,45){\Vars}
\rput(10,25.62){$\addjoin$}
\psline[linewidth=0.65](70,45)(120,45)
\psline[linewidth=0.65](70,5)(120,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(123.75,40)(123.75,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](75,31.25)(75,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](66.25,40)(75,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(75,18.75)(66.25,10)
\psline[linewidth=0.65](117.5,46.25)(120,45)
\psline[linewidth=0.65](70,5)(72.5,3.75)
\rput(125,45){\Vars}
\rput(125,5){\Vals}
\rput(70,25.62){$\addjoin$}
\psline[linewidth=0.65](130,45)(180,45)
\psline[linewidth=0.65](130,5)(180,5)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(183.75,40)(183.75,10)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](135,31.25)(135,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](126.25,40)(135,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(135,18.75)(126.25,10)
\psline[linewidth=0.65](177.5,46.25)(180,45)
\psline[linewidth=0.65](130,5)(132.5,3.75)
\rput(185,45){\Vars}
\rput(185,5){\Vals}
\rput(130,25.62){$\addjoin$}
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,45)(210,45)
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,5)(210,5)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](195,31.25)(195,18.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](186.25,40)(195,31.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(195,18.75)(186.25,10)
\rput(190,25.62){$\addjoin$}
\psline[linewidth=0.65](10,120)(60,120)
\psline[linewidth=0.65](10,80)(60,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(63.75,115)(63.75,85)
\rput(5,135){\Alce}
\rput(65,135){\Bobo}
\rput[b](35,121.25){$\Request$}
\rput[b](35,81.25){$\Response$}
\rput[r](62.5,100){$\Bobsresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](15,106.25)(15,93.75)
\rput[r](2.5,100){$\Alceresource$}
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](6.25,115)(15,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(15,93.75)(6.25,85)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(3.75,115)(3.75,85)
\psline[linewidth=0.65](57.5,121.25)(60,120)
\psline[linewidth=0.65](10,80)(12.5,78.75)
\rput[l](16.25,100){$\Alcebobsresource$}
\rput(65,120){\Vars}
\rput(5,80){\Vals}
\rput(65,80){\Vals}
\rput(5,120){\Vars}
\rput(10,100.62){$\addjoin$}
\psline[linewidth=0.65](70,120)(120,120)
\psline[linewidth=0.65](70,80)(120,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(123.75,115)(123.75,85)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](75,106.25)(75,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](66.25,115)(75,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(75,93.75)(66.25,85)
\psline[linewidth=0.65](117.5,121.25)(120,120)
\psline[linewidth=0.65](70,80)(72.5,78.75)
\rput(125,120){\Vars}
\rput(125,80){\Vals}
\rput(70,100.62){$\addjoin$}
\psline[linewidth=0.65](130,120)(180,120)
\psline[linewidth=0.65](130,80)(180,80)
\psline[linewidth=0.65,arrowsize=1.55 2,arrowlength=1.5,arrowinset=0]{->}(183.75,115)(183.75,85)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](135,106.25)(135,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](126.25,115)(135,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(135,93.75)(126.25,85)
\psline[linewidth=0.65](177.5,121.25)(180,120)
\psline[linewidth=0.65](130,80)(132.5,78.75)
\rput(185,120){\Vars}
\rput(185,80){\Vals}
\rput(130,100.62){$\addjoin$}
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,120)(210,120)
\psline[linewidth=0.65,linestyle=dotted,dotsep=4](190,80)(210,80)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](195,106.25)(195,93.75)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2](186.25,115)(195,106.25)
\psline[linewidth=0.65,linestyle=dashed,dash=2 2,arrowsize=1.5 2,arrowlength=1.5,arrowinset=0.05]{->}(195,93.75)(186.25,85)
\rput(190,100.62){$\addjoin$}
\end{pspicture}


==> PICS/wave.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Nov 10 13:45:14 GMT 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-3.36" x-max="75" y-min="4.96" y-max="48.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.65"
%	 fill-style= "none"
%	 points= "(42.5,11.88);(42.5,11.88);(68.12,23.12);(68.12,23.12)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.65"
%	 fill-style= "none"
%	 points= "(42.5,43.12);(42.5,43.12);(68.12,26.88);(68.12,26.88)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.65"
%	 fill-style= "none"
%	 points= "(10.5,25);(10.5,25);(36.88,11.88);(36.88,11.88)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-width= "0.65"
%	 fill-style= "none"
%	 points= "(11.25,26.25);(11.25,26.25);(36.88,43.12);(36.88,43.12)"
%	 arrow-global-scale-length= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 />
%<circle p3= "(61.88,30.62)"
%	 p2= "(63.12,25.62)"
%	 p1= "(61.25,20)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(15.62,28.75)"
%	 p2= "(16.88,25.62)"
%	 p1= "(15.62,22.5)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(21.53,32.5)"
%	 p2= "(23.75,25)"
%	 p1= "(22.5,19.38)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(28.08,36.63)"
%	 p2= "(31.88,26.25)"
%	 p1= "(28.75,16.25)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(34.38,41.25)"
%	 p2= "(40.62,26.88)"
%	 p1= "(35.62,12.5)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(43.75,42.5)"
%	 p2= "(50,27.5)"
%	 p1= "(43.75,12.5)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<circle p3= "(54.84,35.03)"
%	 p2= "(57.5,26.25)"
%	 p1= "(53.75,16.88)"
%	 closure= "open"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(11.5,27)"
%	 p2= "(11.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(8.5,23)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(41.5,12)"
%	 p2= "(41.5,8)"
%	 fill-color= "#ff6666"
%	 p1= "(38.5,8)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(71.5,27)"
%	 p2= "(71.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(68.5,23)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(41.5,47)"
%	 p2= "(41.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(38.5,43)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(75,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%\Carol
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(6.25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%\Alice
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(40.62,48.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Bob
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(40,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\Dave
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(75,48.75)
\psline[linewidth=0.65,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(42.5,11.88)(68.12,23.12)
\psline[linewidth=0.65,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(42.5,43.12)(68.12,26.88)
\psline[linewidth=0.65,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(10.5,25)(36.88,11.88)
\psline[linewidth=0.65,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(11.25,26.25)(36.88,43.12)
\rput{0}(53.18,25.81){\psellipticarc[](0,0)(9.95,9.95){-35.73}{28.94}}
\rput{0}(12.37,25.62){\psellipticarc[](0,0)(4.51,4.51){-43.92}{43.92}}
\rput{0}(10.19,25.07){\psellipticarc[](0,0)(13.56,13.56){-24.8}{33.26}}
\rput{0}(15.13,26){\psellipticarc[](0,0)(16.75,16.75){-35.6}{39.37}}
\rput{0}(19.39,26.2){\psellipticarc[](0,0)(21.24,21.24){-40.18}{45.11}}
\rput{0}(28.88,27.5){\psellipticarc[](0,0)(21.12,21.12){-45.24}{45.24}}
\rput{0}(42.95,26.64){\psellipticarc[](0,0)(14.55,14.55){-42.1}{35.23}}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(10,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(40,10){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(70,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(40,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\rput[l](75,25){\Carol}
\rput[r](6.25,25){\Alice}
\rput[b](40.62,48.75){\Bob}
\rput[t](40,5){\Dave}
\end{pspicture}

